Uncertainty-Induced Transferability Representation for Source-Free Unsupervised Domain Adaptation

Source-free unsupervised domain adaptation (SFUDA) aims to learn a target domain model using unlabeled target data and the knowledge of a well-trained source domain model. Most previous SFUDA works focus on inferring semantics of target data based on the source knowledge. Without measuring the transferability of the source knowledge, these methods insufficiently exploit the source knowledge, and fail to identify the reliability of the inferred target semantics. However, existing transferability measurements require either source data or target labels, which are infeasible in SFUDA. To this end, firstly, we propose a novel Uncertainty-induced Transferability Representation (UTR), which leverages uncertainty as the tool to analyse the channel-wise transferability of the source encoder in the absence of the source data and target labels. The domain-level UTR unravels how transferable the encoder channels are to the target domain and the instance-level UTR characterizes the reliability of the inferred target semantics. Secondly, based on the UTR, we propose a novel Calibrated Adaption Framework (CAF) for SFUDA, including i)the source knowledge calibration module that guides the target model to learn the transferable source knowledge and discard the non-transferable one, and ii)the target semantics calibration module that calibrates the unreliable semantics. With the help of the calibrated source knowledge and the target semantics, the model adapts to the target domain safely and ultimately better. We verified the effectiveness of our method using experimental results and demonstrated that the proposed method achieves state-of-the-art performances on the three SFUDA benchmarks. Code is available at https://github.com/SPIresearch/UTR.

==> samples/method.tex <==




\begin{figure*}[t]
  \centering

  
   \includegraphics[width=0.6\linewidth]{figs/method.png}
   \caption{Overview of our “inherit-calibrate-discover” framework. In the Inherit step, we measure the \textit{Domain Distributional Representation Uncertainty} of the source feature $DDRU(h_s)$, and use it to estimate the transferability of the source feature $z_s$. Then we distill $z_s$ into the target encoder $h_t$ with $L_{kd}$, which is controlled by $DDRU(h_s)$ to select transferable knowledge. In the Calibrate step, we first select samples with high \textit{Inference Risk Index} . Then we calibrate their prediction \lisays{in} a forget-discover manner. The forget loss $L_{f}$ pushes the prediction distribution of these samples to be uniform to each category, forcing the model to forget the current prediction. Then the discover loss $L_{d}$ guides it to discover the true category. Leveraging the above two steps, the target model ``safely'' integrates the source knowledge and finally \lisays{adapts} to the target domain with the adapt loss $L_{a}$. }
   \label{fig:method}
  
\end{figure*}

\section{Method}
%This section introduce our method. 
%For better illustration, we first details the proposed Domain Distributional Representation Uncertainty and its derivatives, the transferability index and the inference risk index in Sec. \ref{sec:DDRU}. Then, we demonstrate the whole "inherit-calibrate-discover" framework in \ref{sec:ica}.

\subsection{Overall}

In this paper, we focus on the K-way visual object classification task. 
In SFUDA, a source model $f_{s}$ is firstly trained on the source domain $D_S$ represented by $f_{s}=g_{s} \circ h_{s}$, where $h_{s}$ is the feature extractor, and $g_{s}$ is the classifier. The target domain $D_t=\{x_t^i\}_{i=1}^{n_t}$ consists of $n_t$ unlabeled samples. The SFUDA aims to learn a discriminative target model $f_t= g_{t} \circ h_{t}$ using the source model $f_s$ and unlabelled target data $D_t$.


To measure the transferability of the source model features to the target domain in the absence of source data and target annotations, in Section \ref{sec::DDRU}, we propose a novel measurement termed as the Domain Distributional Representation Uncertainty (DDRU). DDRU integrates the distributional uncertainty of the source features $z \sim \mathbb{R}^{d}$ extracted by the source encoder $h_s$, and generates a $d$-dimension vector $DDRU(h_s)$ to estimate the source feature transferability. Each dimension (the $i^{th}$ as an example) $DDRU(z_i,h_s)$ reveals how transferable the $i^{th}$ feature $z_i$ is: the lower value indicates the higher transferability, and the vice versa.

To facilitate the transferability estimation and adaptation using DDUR, in Section \ref{sec::ica}, we proposed a novel “inherit-calibrate-adapt” (ICA) framework to solve SFUDA in Figure \ref{fig:method}, comprising of the \textit{Inherit}, the \textit{Calibrate} and finally the \textit{Adapt}.
Specifically, \textbf{in the \textbf{inherit} step}, the target model $f_t$ inherits the transferable feature representations (identified by DDRU) from the source model  $f_t$ by minimizing a transferability-induced knowledge distillation loss $\mathcal{L}_{kd}$. Different from the conventional knowledge distillation, we are able to control the distillation process using the quantified transferability $DDRU(h_s)$ by assigning more transferable features a larger weight. $\mathcal{L}_{kd}$ prompts the target domain model to learn transferable source feature representations.

%The quantified knowledge distillation promotes inheriting transferable features from $h_s$ to the target encoder $h_t$.
%In this paper, we focus on the knowledge contained in the source encoder $h_s$. 
%We first propose the Domain Distributional Representation Uncertainty (DDRU) module to estimate the transferability of $h_s$ by producing a $d$-dimension vector $DDRU(h_s)$, each of its dimensions representing how transferable that dimension is. Then, 

%The source representations learned from source data may be deficient for target domain data. We still need to learn target-specific representation based on the inherited representations. To this end, we propose to infer the category of the target data $\hat{y}$ based on the inherited knowledge. %Given $x_t$, the inferred category is $\hat{y}=\arg\max_y P(y|x_t)$, where $p(y|x_t)=\sigma( g_{t;\theta_g} \circ h_{t;\theta_h}(x_t))$, $\sigma$ is the softmax function. 
%However, due to the cross-domain discrepancies, there is a risk in adapting the model using the inferred category information.

%After inheriting the knowledge from the source model, we obtained a target model $f_t=g_t \circ h_t$. \chensays{why is it useful here?}
\textbf{In the \textbf{calibrate} step}, we further alleviate the risk of the less-transferable representations by calibrating the predictions. We proposed the \textit{Inference Risk Index} (IRI) to detect the risk of target samples whose predictions are mainly inferred by the less-transferable features. Specifically, we first measure the transferability of each target feature using the $DDRU(h_t)$. Then,  the target model predicts the category of the input data $x_t$ belongs to the $k^{th}$ class and we propose to 
trace the contribution of each feature to infer $k$, denoted as $CTR(x_t,k,z)$. Finally, we propose to calculate the IRI using the dot product of $DDRU(h_t)$ and $CTR(x_t,k,z)$. A small IRI value $IRI(x_t)$ represents that the model prediction of $x_t$ is mainly attributed to the transferable features and the prediction of this sample is reliable; while a large value indicates the prediction is inferred by less-transferable features and using this sample to update model brings risks. 

After identifying the risk samples, we focus on calibrating the prediction of the high-risk samples. Without target annotations as supervision, we need to discover their true categories using the model only. As the predictions inferred by less-transferable features are prone to be wrong, we propose a loss function $L_f$ to \textit{forget} the current predictions by regularizing the prediction distributions to be uniform across multiple classes. 
Then, incorporating reliable category information of low-risk samples, we guide the model to discover the true categories of the high-risk samples by forcing their prediction close to a certain class with the discovery loss $L_d$. Such a "forget-discover" process helps the model to free itself from the shackles of less-transferable knowledge, thus facilitating the discovery of its true categories.

Leveraging the above two steps, the target model ``safely'' integrates the source knowledge. The "adapt" step \textit{\textbf{finally}} refines the target model using inferred supervisions from the transferable knowledge, therefore summarizing a better-performing discriminative model.


%The \textbf{calibrate} step calibrates the inherited knowledge by calibrating the inferred categorical information, which can further discard the negative influence of non-transferable source knowledge. 



%First, we introduce the \textit{Inference Risk Index} (IRI) to estimate the per-sample risks using the inherited source knowledge for inference. \chensays{how? we need to be specific-ish about it here.} The intuition is that the inference of a sample is reliable if it is based on the transferable knowledge, and it is risky if not.
%Next, we design a novel strategy to calibrate the inferred category of samples with high IRI, by first forgetting the current inference and then discovering the true category. 

%\textbf{\textit{The Adapt Step:}} based on the above preparations, we finally integrate the transferable source knowledge and discard the non-transferable one. Then we can adopt the model to the target domain by refining the model with target data and the inferred category.

\subsection{Domain Distributional Representation Uncertainty}
\label{sec::DDRU}
To inherit transferable knowledge from the source model, an essential question is: How to identify the transferability of the source knowledge to the target domain in SFUDA?
Our solution is motivated by the distributional uncertainty \cite{malinin2018predictive,gawlikowski2021survey,nandy2020towards}.

\noindent\textbf{Background of distributional uncertainty and motivations:} Given an annotated sample $(x,y)$ and a model $\theta$ trained on \lisays{a} domain $D$, the distributional uncertainty is in the second part of the following uncertainty factorization:
{\setlength\abovedisplayskip{1pt}
\setlength\belowdisplayskip{1pt}
\begin{equation}
P(y|x,D)= \iint  \underbrace{P(y|\mu)}_{Data} \underbrace {P(\mu|x,\theta)}_{Distributional} \underbrace {P(\theta|D)}_{Model}d\theta d\mu,
\label{eqa:uncertainty}
\end{equation}}
where $\mu$ is the predicted label distribution. \textit{The distributional uncertainty reveals the uncertainty of whether $x$ is from its potential training data distribution $D$ of the model.} With the uncertainty measurement function $M(\cdot)$ \cite{kendall2017uncertainties,gal2016dropout,lakshminarayanan2016simple}, we denote the measured distributional uncertainty as $M(x,\theta)$ ($\mu$ is 
generally inferred by $x$ and $\theta$). This effect provides us \lisays{with a} a new perspective to understand and measure the transferability. Considering to predict a target sample $x=x_t$ using the source model $\theta=\theta_s$, a low distributional uncertainty demonstrates that the target sample $x_t$ is ``close'' to the source domain $D_s$ given a source model $\theta_s$. This reflects that it is efficient for the model $\theta_s$ to reduce the domain discrepancy between the target and source domain, suggesting the source model is transferable to the target distribution. Similarly, high distributional uncertainty denotes the model is less transferable. Therefore, we are inspired to leverage the distributional uncertainty to estimate the transferability.

Leveraging the distributional uncertainty, we modify it to fit the SFUDA and propose the Domain Distributional Representation Uncertainty (DDRU) to address the challenges in the SFUDA task. 

\textit{First}, the previous distributional uncertainty evaluates the whole model over the target instance and the source distribution. Since SFUDA provides a well-trained source model, we aim to explore the transferability of the \textit{partial} knowledge within the source model. It is useful and necessary to determine which knowledge is transferable to the target domain, rather than directly using the whole model. To this end, we decompose the distributional uncertainty by the following:
{\setlength\abovedisplayskip{1pt}
\setlength\belowdisplayskip{1pt}
\begin{equation}
\begin{aligned}
P(\mu|x_t,\theta_s) \approx \sum_{i=1}^d P(\mu|z_i,g_{s;\theta_{gs}}) P(z_i|x_t,h_{s;\theta_{hs}}),
\end{aligned}
\label{eqa:decompose}
\end{equation}}
where  $z=h_s(x)$ is the $d$-dimension feature representations and $z_i=h_s^i(x)$ is the feature representation at the $i^{th}$ dimension. It is assumed that there is little uncertainty in the term $P(\mu|z_i,g_{s})$, based on the theoretical results that the $g_{s}$ is closely related to the optimal target classifier  \cite{kuzborskij2013stability, liang2020we}.
Therefore, we approximate the distributional uncertainty by measuring the uncertainty of each dimensional  feature representation $P(z_i|x_t,h_{s})$, denoted by $M^i(x_t,h_{s})$, and obtained a $d$-dimension vector, $M(x_t,h_{s})=[M^1(x_t,h_{s}),..., M^d(x_t,h_{s})]$.
It is straight-forward that the $i^{th}$ dimension value $M^1(x_t,h_{s})$ represents the uncertainty of $z_i$, and thus can estimate the transferability of $z_i$. 

Second, the previous distributional uncertainty represents the uncertainty of a sample to a domain distribution.
In SFUDA, we are more interested in capturing the uncertainty between the whole target domain and the source domain. To this end, we propose to model the distributional uncertainty between the two domains by calculating the expectation of $M(x_t,\theta)$ by integrating $x_t$ over the target domain $D_t$, and develop the Domain Distributional Representation Uncertainty (DDRU):

{\setlength\abovedisplayskip{1pt}
\setlength\belowdisplayskip{1pt}
\begin{equation}
\begin{aligned}
DDRU(h_{s})=&[DDRU^1(h_{s}),..., DDRU^d(h_{s})]\\
&=[\mathbb{E}_{x_t \sim \mathcal{X}_t } M^d(x_t,h_{s}),..., \mathbb{E}_{x_t \sim \mathcal{X}_t } M^d(x_t,h_{s})]

\end{aligned}
\label{eqa:DDRU}
\end{equation}}

 Out of various methods to measure the uncertainty \cite{kendall2017uncertainties,gal2016dropout,lakshminarayanan2016simple}, we adopt the sensitivity analysis method \cite{nagy2007distributional} as $M(\cdot)$ in this paper due to its computational efficacy. To be specific, the model parameters of $h_s$ are perturbed for $T$ times randomly as follows: $\{\theta_{hs;T}=(1+r_t)*\theta_{hs}\}_{t=1}^T$ are \textit{firstly} calculated by inserting $T$ random perturbations $\{r_t\}_{t=1}^T$ to original parameter $\theta_{hs}$; \textit{Then} the uncertainty is estimated by calculating the variance of the $T$ outputs of the $i^{th}$ dimension feature:
{\setlength\abovedisplayskip{1pt}
\setlength\belowdisplayskip{1pt}
\begin{equation}
   M^i(x_t,h_{s})= Var_{\theta_{hs}\sim\theta_{hs;T}}(h_{\theta_{hs}}^i(x_t)). 
  \label{eqa:mDDRU}
  \vspace{-3mm}
\end{equation}}

\subsection{Inherit-Calibrate-Adapt Framework}
\label{sec::ica}
\noindent\textbf{The Inherit Step:} Given the source encoder $h_{s}$, we extract the target domain representations $z = h_{s}(x_t)$.
Then the $DDRU(h_{s})$ is calculated following the Equation.\eqref{eqa:DDRU} to estimate the transferability of each feature in $z$, where a lower $DDRU$ value suggests stronger transferability. 
Then, the target model inherits the source knowledge based on the identified transferability. We proposed a novel transferability-induced knowledge distillation loss as follows: 
\begin{equation}
L_{kd}=\mathbb{E}_{x_t\sim \mathcal{X}_t}  [ \Vert Q(DDRU(h_{s})) \odot [h_{s}(x_t)- h_{t;\theta_{ht}}(x_t)]\Vert_2],
\end{equation}
where $Q(x)=sigmoid(-x)$ is a monotone minus function, $\odot$ is the Hadamard product\chensays{what is dot product? between element wise? or scalar product}. The mean squared error loss $\Vert h_{s}(x_t)- h_{t;\theta_{ht}}(x_t)\Vert_2$ is modified to distill knowledge within $h_s$ to $h_t$ in a reweighted manner and our proposed DDRU $Q(DDRU(h_{s}))$ calculates the adjusted weights. The aim is to assign large weights to \lisays{dimension} with low $DDRU$ while small ones to those with high $DDRU$, guiding the target model to inherit more transferable knowledge from the source model in a well-controlled manner.



%The \textit{Calibrate Step} focuses on calibrating the inferred category information before the later \textit{Adapt Step}.
%We first propose the \textit{Inference Risk Index} (IRI) to estimate the risk of leveraging the inferred category.
%Then, we select high IRI samples and calibrate their inferred category with a novel "forget-discover" strategy.

% and can use it to infer target samples' category.
%For $x_t$  the inferred category by classifier $g$ is $k=\arg\max_y \hat{y}$, where $\hat{y}=g(z)$ is the predicted logit, $z\sim \mathbb{R}^{d}$ is the extracted representation and $g$ is the classifier. 
\noindent\textbf{The Calibrate Step:} In \textit{the calibrate step}, we aim to calibrate the risk predictions caused by less-transferable features, therefore eliminating their negative effects when updating the target model $f_t$.
To this end, we first propose a new metric termed as \textit{Inference Risk Index}(IRI) to detect the risk of target samples whose \lisays{predictions} are made by less-transferable features. \chensays{The IRI is composed of two parts, including }


Specifically,
given a target sample $x_t$, its predicted category by the target model is $k=\arg \max \sigma(f_t(x_t))$, where $\sigma(.)$ is the softmax function and $\sigma(f_t(x_t))$ is the predicted probability distribution. Note that we denote $\sigma(f_t(x_t))$ as $p(x_t)$ for simplicity.
IRI estimates the inference risk by tracing which features mainly determine the prediction, and whether they are transferable. 
We first estimate the contribution of each dimension representation $\{z_i\}_{i=1}^d$ in inferring $x_t$ to the $k$ by:
{\setlength\abovedisplayskip{1pt}
\setlength\belowdisplayskip{1pt}
\begin{equation}
CTR(x_t,k,z)=\sigma(\left|\frac{\partial p^k(x_t)}{\partial z}\right|),
\label{eqa:ctr}
\end{equation}}
where $p^k(x_t)$ is the probability to $k$ category, $z=h_t(x_t)$ the model output to the $k^{th}$ category. 

\peisays{To explicitly understand,  CTR first  calculate the   the partial derivative of $p^k(x_t)$  wrt. each of the $d$ dimension features $z=[z_1,...,z_d]$, which denotes the trend of the $p^k(x_t)$ to the change of each $z_i$. 
 If its $i^{th}$ dimension value is close to $0$, the $P^{k}(x_t)$ is unsensitive with the change of $z_i$, which suggests the prediction is not determined by $z_i$.
In contrast, the current prediction $k$ is mainly come from those $z_i$ that $P^{k}(x_t)$ are sensitive with.
Therefore, we can capture sensitivity with the absolute value of the partial derivative term, and use $\sigma$ to normalize it as the contribution of each feature in getting $k$.}
\peisays{I think the expression is not clear}


Then, we use our DDDRU  to estimate the transferability of each dimension feature $z_i$, producing the vector $DDRU(h_{t})$.
Finally, the \textit{Inference Risk Index} is calculated by the dot product between the two term.
{\setlength\abovedisplayskip{1pt}
\setlength\belowdisplayskip{1pt}
\begin{equation}
IRI(x_t,h_{s})=CTR(x_t,k,z) \cdot DDRU(h_{t})
\label{eqa:iri}
\end{equation}}

 %The expected knowledge should be able to assign clear and correct semantic information to target data. 
%Let $p(x_t)$ denote the model prediction distribution, i.e. $p(x_t)=\sigma( g_{t;\theta_g} \circ h_{t;\theta_h}(x_t))$, where $\sigma$ is the softmax function.

We leverage IRI to detect high risk samples that satisfy $\{x_t:IRI(x_t)>\tau_r\}$ as $\mathcal{X}_{t;HIRI}$, where $\tau_r$ denote the threshold.
In the following, we focus on calibrating the model prediction of these samples.  %, on which the knowledge from the source domain is prone to make a false prediction. These hard samples reveal the discrepancy between source-learned and target-specific knowledge, which plays an important role in adapting the model to the target domain.   
%The high IRI indicates that the knowledge from the source model are prone to make false inference on these samples.
Without any target annotation as supervision, we can only discover the potential true label by the model itself.
However, self-discovering categories based on the current model are, on the other hand, constrained by the model, especially when the model is confident in its wrong predictions. Therefore, it is difficult to directly self-discover the true information.
To this end, we propose to first  increase the entropy of the prediction probability distribution, which pushes the distribution uniform to each category, thus forgetting the current knowledge and freeing from its  constraint. The forget loss $L_f$ is formulated as.
{\setlength\abovedisplayskip{1pt}
\setlength\belowdisplayskip{1pt}
\begin{equation}
%\begin{aligned}
    L_{f} =\mathbb{E}_{x_t \sim \mathcal{X}_{t;HIRI} }\sum_{k=1}^K p(x_t) log p(x_t)),
        %\\&+  \sum_{k=1}^K  p^k log p^k;
%\end{aligned}
\end{equation}}
where $p(x_t)=\sigma(f_t(x_t))$ is the prediction probability distribution of $x_t$.
As illustrated in Figure \ref{fig:method}, increasing the entropy makes the prediction probability distribution of the target domain model uniform and thus can get rid of  the  constraint of source knowledge.

After the "forget" is done, we guide the target model to discover the true category of the target sample by inferring the prediction into a certainty category.  The the \lisays{discovery} loss $L_d$ is : 
{\setlength\abovedisplayskip{1pt}
\setlength\belowdisplayskip{1pt}
\begin{equation}
%\begin{aligned}
    L_{d} = -\mathbb{E}_{x_t \sim \mathcal{X}_{t} }\sum_{k=1}^K p(x_t) log p(x_t))%\sum_{k=1}^K \sigma(f_t (x_t)) log \sigma(f_t (x_t)).
        %\\&+  \sum_{k=1}^K  p^k log p^k;
%\end{aligned}
\end{equation}}
$L_d$ aims to minimize the entropy of the prediction probability distribution, forcing the model to assign the prediction to a certainty class.
Note that, instead of only minimizing the entropy of $\mathcal{X}_{t;HIRI}$, we put $\mathcal{X}_{t;HIRI}$ back into $\mathcal{X}_{t}$ to reduce the entropy of $\mathcal{X}_{t}$. In this case, the semantic information of samples with \textit{Inference Risk Index}, which the model relatively correctly extracts, can be introduced to help the category discovery of $\mathcal{X}_{t;HIRI}$.

To avoid the degenerated solution of the entropy minimizing  that the model \lisays{assigns} all data as some specific classes, we adopt the prediction diversity loss which is widely used in clustering \cite{jabi2019deep,ghasedi2017deep} and domain adaptation works \cite{liang2020we,yang2021exploiting}.
{\setlength\abovedisplayskip{1pt}
\setlength\belowdisplayskip{1pt}
\begin{equation}
%\begin{aligned}
    L_{div} =KL(\overline{p}||q ),
        %\\&+  \sum_{k=1}^K  p^k log p^k;
%\end{aligned}
\end{equation}}
where $\overline{p}=\mathbb{E}_{x_t \sim \mathcal{X}_{t}}\sigma(g_{t;\theta_g} \circ h_{t;\theta_h} (x_t)$ and $q_{\{k=1,...K\}}=\frac{1}{K}$ is a uniform distribution.
%Since the low-risk samples in $\mathcal{X}_{t}$ that have relatively accurate semantic extraction the model can support the semantic discover of $. 

\begin{algorithm} 
\caption{ algorithm}
\label{algorithm}
%\hspace*{0.02in} 
\begin{algorithmic} 
\REQUIRE $f_{s;\theta}=g_{s} \circ h_{s}$, $f_{t;\theta}=g_{t} \circ h_{t}$,$D_t$ 

\REQUIRE hyperparameter $\tau_r$, $\lambda_1$,$\lambda_2$
%\REQUIRE $X_t$ 
%\REQUIRE $\tau_{hi},\tau_{li},\tau_p,\gamma,\lambda_1,\lambda_2$ 

%\STATE Initialize f_{t;\theta} by f_{s;\theta}
%\STATE fixed g_{t;\theta_g}
%\FOR{$x$ $\in$ $range(1,K)$}
%\STATE {$F_i$ $\gets$ Perturb($F$)}
%\ENDFOR
Calculate $DDRU(h_s)$
\WHILE{not done}\\
\STATE Sample batch $T$ from $D_t$ \\
\STATE Update $g_t$ to inherit knowledge from $f_t$ by optimizing $\lambda_1 L_{KD}$
\STATE Select high risk samples that $IRI(x_t)>\tau_r$
\STATE Update $f_t$ to discard source constraint by optimizing $\lambda_2 L_{f}$
\STATE Update $f_t$ to discover  by optimizing $L_{d}+L_{div}$
\STATE Update $f_t$ to adapt by optimizing $L_{a}$
%\STATE Split dataset into four parts according to $DRU_(x_t),\tau_{hi},\tau_{li},\tau_p$.
%\STATE Inherit: distill transferable representations from $h_{s}$ to $h_{t;\theta_h}$ via $DRU_(z)$.
%\STATE Calibrate inherited knowledge by Equation \ref{}.
%\STATE Discover new knowledge by Equation \ref{}.

%\STATE Self-discover based on the support set
\ENDWHILE 
\end{algorithmic}  
\end{algorithm}
%We argue that target class predictions of these data reflect the effect of negative transferable representations.
%The ideal way to calibrate these predictions is to optimize the model's predictions with the ground-truth labels. However, without the target annotations, we alternatively propose to minimize the negative cross-entropy loss for optimizing those data, in order to suppress the role of negative transferable representations. This procedure proves effective for mining their true class information by self-discovery (the next Adapt step). The loss for $\mathcal{X}_{t;3}$ is:

%\peisays{I'm revising  this section}


%We select “easy-to-adapt” samples by select $\{x_t:max(p(x_t))>\tau_p\}$, where $\tau_p$ is a threshold.
%Then we split these selected samples to three parts according to their identifiability index using two threshold $\tau_{hi}$ and $\tau_{li}$: identifiable samples $\mathcal{X}_{t;1}=\{x_t:I(x_t)\geq\tau_{hi}\}$, middle identifiable samples  $\mathcal{X}_{t;2}=\{x_t:\tau_{hi}>I(x_t)\geq\tau_{li}\}$ and unidentifiable samples  $\mathcal{X}_{t;3}=\{x_t:I(x_t)>\tau_{li}\}$.
%For samples with unclear model predictions (i.e. the prediction distribution with high-entropy), it is hard to determine whether it is caused by inheriting negative transferred features or the deficient knowledge. To this end, \textit{C-Step} only focuses on samples whose prediction distribution is with low-entropy, aiming to calibrate the inherited representation by calibrating the predicted class information of the model to these data.

%As analysed in Section \ref{3.3}, the prediction accuracy correlates with the $I(x_t)$. Therefore, we split the low entropy samples into three sets: identifiable samples with low $I(x_t)$ $\mathcal{X}_{t;ld}$, middle identifiable samples with  middle $I(x_t)$ $\mathcal{X}_{t;md}$ and not identifiable samples with high $I(x_t)$ $\mathcal{X}_{t;hd}$.

%For the samples in $\mathcal{X}_{t;1}$, the predictions of the model can be trusted. 
%Therefore, we can directly use the model prediction as its pseudo label to enhance the effectiveness knowledge in the model.
%The objective  can be formulated as:
%{\setlength\abovedisplayskip{1pt}
%\setlength\belowdisplayskip{1pt}
%\begin{equation}
%    L_{c1}=\mathbb{E}_{x_t \sim \mathcal{X}_{t;1} } L_{CE}(x_t,y^p).
%\end{equation}}
%where $L_{CE}$ is the widely used cross-entropy loss,  $y^p=argmax(p(x_t))$ is the label of the category in which the maximum value of the model's predicted probability distribution.

%For samples in $\mathcal{X}_{t;2}$, we introduce a identifiability-rectified label,  which aims to selectively strength prediction for samples according to their $I(x_t)$. For $x$ whose prediction distribution is $p(x_t)$, the middle enhance label is:
%{\setlength\abovedisplayskip{1pt}
%\setlength\belowdisplayskip{1pt}
%\begin{equation}
%  y^{me}=  p(x_t)^{ \frac{I(x_t)}{\gamma} }/\sum_{j=1}^{K}p_j(x_t)^{\frac{I(x_t)}{\gamma}},
%\end{equation}}
%where $\gamma$ is a scaling coefficient, $p_j(x_t)$ is the $j$-th class probability of the prediction. Note that the pseudo-label we used for $\mathcal{X}_{t;1}$ can be regard as a specific case of identifiability-rectified label if $\gamma \rightarrow \infty$.
%With calibrated label, the loss for $\mathcal{X}_{t;2}$ is:
%{\setlength\abovedisplayskip{1pt}
%\setlength\belowdisplayskip{1pt}
%\begin{equation}
%L_{c2}= \mathbb{E}_{x_t \sim \mathcal{X}_{t;2} } L_{CE}(x_t,y^{me}).
%\end{equation}}
%With low identifiability index, the feature representations are prone to make false prediction for samples in $\mathcal{X}_{t;3}$.  We argue that target class predictions of these data reflect the effect of negative transferable representations.
%The ideal way to calibrate these predictions is to optimize the model's predictions with the ground-truth labels. However, without the target annotations, we alternatively propose to minimize the negative cross-entropy loss for optimizing those data, in order to suppress the role of negative transferable representations. This procedure proves effective for mining their true class information by self-discovery (the next Adapt step). The loss for $\mathcal{X}_{t;3}$ is:
%On the one hand, the negative cross-entropy can leverage the information that the current predictions  are wrong with high probability, and  steers the model away from current predictions. On ther other hand, it can lead the model to make a high entropy prediction, which makes preparation for the model to get rid of the existing predictions and discover the class information of these samples. The negative cross-entropy loss is:
%{\setlength\abovedisplayskip{1pt}
%\setlength\belowdisplayskip{1pt}
%\begin{equation}
%    L_{c3}=-\mathbb{E}_{x_t \sim \mathcal{X}_{t;3} } L_{CE}(x_t,y^p).
%\end{equation}}

%\vspace{-3mm}
%We first analyze two extreme cases.  For samples in $\mathcal{X}_{t;ld}$,  the representation of the model is robust to those samples, and  is close to one certain class prototype, indicating the predictions of the model  trusted. 
%The final loss in the calibrate step can be summarized as:
%{\setlength\abovedisplayskip{1pt}
%\setlength\belowdisplayskip{1pt}
%\begin{equation}
%L_{cal}= L_{c1}+L_{c2}+L_{c3}.
%\end{equation}}

\noindent\textbf{The Adapt Step:} 
In \textit{the adapt step}, we finally \lisays{leverage} the knowledge integrated by the above two steps to infer the target category, and \lisays{use} it to refine the target model, thus adapting to the target \lisays{domain}. The category inference can be easily performed by most previous SFUDA methods\cite{liang2020we, yang2021generalized, yang2021exploiting,li2021imbalanced,xia2021adaptive}, which is not our focus. In this paper, we adopt the pseudo-label strategy in \cite{liang2020we} consider its simplicity and effectiveness.
Specifically, given a target samples $x_t$, we infer the categories of the samples following  \cite{liang2020we}, and denote it as the pseudo-label $y_t$ of $x_t$. Then we can refine the model with the cross-entropy loss:

\begin{equation}
%\begin{aligned}
   L_{a}= \mathbb{E}_{x_t \sim \mathcal{X}_{t} } CE(x_t,y_t).
%\end{aligned}
\end{equation}

%\noindent\textbf{Overall Formulation and Optimization}
%We iteratively perform the three step with some coefficient to control the losses, including $\lambda_1$ for $L_{kd}$ and $\lambda_2$ for $L_{f}$. . The overall objectives are as follows.

%In the inherit step:
%\begin{equation}
%    \min_{h_t} \lambda_1 L_{KD}.
%\end{equation}

%In the calibrate step, first:
%\begin{equation}
%    \min_{f_t} \lambda_2  L_{f}.
%\end{equation}

%then:
%\begin{equation}
    \min_{f_t}L_{d}.
%\end{equation}

%In the adapt step:
%\begin{equation}
%    \min_{f_t}L_{a}.
%\end{equation}


% Regardless of the correctness, the target model inheriting the source domain knowledge is able to predict a  class distribution for  samples by metric the similarity between the class prototype contains in the classifier and feature representation extrated by the feature encoder. 
% \begin{equation}
%     p(x_t)= g_{s} \circ h_{s}(x_t).
% \end{equation}
% If the representation is close to one certain class prototype,  the model will give a clear class   information to the samples, which is reflected by the low entropy of the predicted distribution $p(x_t)$.
% The predicted class   information can guide to mine their own true category semantics.  
% However, due to the domain gap, the representation extracted from the model may be loss its  semantic information. In this case, the predicted class semantic information is prone to be wrong, leading the model to learn in the wrong direction.

% In this step, we  aim to integrate the transferred inherited source domain knowledge, use it to predict target samples with low entropy. and calibrate wrong prediction.
% The main idea is that, we should absorb the predicted class semantic information of a sample conditioned on the robustness of the model to the sample.

% To this end,  we  then expand the feature uncertainty into sample level to measure the robustness of feature to each sample.
% The sample-level feature uncertainty can be calculated by:

% \begin{equation}
% U_{h_{\theta_h}}(x_t)= \sum_{i=1}^d[Var(h(\theta_h,x))_{\theta_h \sim P(\theta_h,D_t)}],
% \end{equation}


% \begin{equation}
%   Calibrate(p(x_t))=  p(x_t)^{\frac{1}{U(x_t)} }/\sum_{j=1}^{K}p(x_t)_j^{\frac{1}{U(x_t)}}
% \end{equation}

% \begin{equation}
% L_{cal}(x_t)= - \sum_{i=1}^{K} p_i log(Calibrate(p_i)),
% \end{equation}




%Our consideration is threefold. First, the source knowledge that learned from a  labeld-riched source domain  contains usable  knowledge for the target domain, which is valuable to some target domain data. For these data,  the source learned knowledge has been able to give accurate prediction.  Mining knowledge from these data is quite easy, 
%Different from previous works that focus on self-discovering a whole-dataset classification structure like feature cluster or low entropy prediction.

%Instead of focusing on the whole target dataset, we investigate this question for each target data since the value of source knowledge on each target data is different.
%Our evaluation considers from two aspect:  robustness and discrimination of representation.
%The discrimination of representation can be received by the prediction entropy since low entropy  indicate the representation is close to a certain class.
%For robustness, 



==> samples/transfer_exp.tex <==



\begin{figure*}[t]
  \centering
  %\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.24\linewidth]{figs/CA.eps}
    %\includegraphics[width=0.24\linewidth]{figs/CP.eps}
    %\includegraphics[width=0.24\linewidth]{figs/CR.eps}
     \includegraphics[width=0.8\linewidth]{figs/fig_tfs.pdf}
    \vspace{-6mm}
   \caption{The experiment of the source trained model on three source$\rightarrow$target tasks: Cl$\rightarrow$Ar, Cl$\rightarrow$Pr and Cl$\rightarrow$Re. The first  figures show the performance of two different representations $z_{low}$ and $z_{high}$ on target domain. The second figure compares the corresponding angle between $z_{low}$ and $z_{high}$. The third and fource  figures calculate the MMD distance and \mathcal{A}-distance between $D_{low}$ and $D_s$, and $D_{high}$ and $D_s$. The last figure show the performance of the model on the  $D_{low}$ and $D_{high}$. }
   \label{fig:DRU_transfer}
   \vspace{-6mm}
\end{figure*}

%In domain adaptation, transferability characterizes the ability of feature representations to bridge the discrepancy across domains\cite{chen2019transferability}, which is also referred to as the invariance of the learned representations across domains\cite{chen2020harmonizing}.
%It is the key to effectively transferring a learning model from the source domain to the target domain via the feature representations.
%Many vanilla UDA methods used to measure the domain discrepancy between features from source and target domain, such as A-distance, H-distance and discrepancy distance, can be regarded as measures of transferability of the feature representations \cite{ibrahim2021newer}. 
%Recently, \cite{chen2019transferability} propose a corresponding angle to explicitly investigate the transferability of feature representations. 
%Previous works in measuring transferability require  a well-trained model in the source domain and labeled target domain data \cite{nguyen2020leep,bao2019information}.
%These vanilla UDA methods, however,  require  to extract the representations of the source data and target data simultaneously, which are not available in SFUDA.
%Although these methods have shown their effectiveness in vanilla UDA, they are unapplicable to SFUDA since they need to extract source features from source data.

%Inspired by \cite{gao2020reducing} which describes the domain discrepancy as to the distributional uncertainty between source and target, we propose to study the transferability of the feature representations through their distributional uncertainty.
%In the following, we model the distributional uncertainty of the representations (Dru), and experimentally analyze its relationship to feature transferability.
%However, in SFUDA, we cannot get the features of the source domain data.
%Therefore, measure the transferability of the representation by compare its extracted features on the two domains is infeasible.
%Inspired by the definition, we rethink the transferability as the robustness of the representation learned from source domain on target domain.
%The robustness, according to \cite{kwon2021repurposing}, can be captured by the uncertainty.
%Although the source data is not available, SFUDA provide a well-trained model in the source domain, which means the information about source domain is embedded on the model. 
%Different from vanilla UDA.
%\subsection{}
%

\subsection{Dru and the Representation Transferability}
\label{sec:3.2}
% \vspace{-1mm}
% From Equation \ref{eqa:esDRU}, we see Dru is related to two variables $z$ and $x_t$, which provide us two ways to understand it.
In this subsection, we introduce and discuss how Dru is used to approximate and measure the representation transferability. The following discussion comprises two parts: the \textit{conjecture} via formula derivation and the \textit{evidence} via experimental results.

\underline{\textbf{\textit{Conjecture:}}} To investigate the effect of Dru on the representation $z$, we propose to calculate the expectation of $D(z,x_t)$ by integrating $x_t$ over the target domain $D_t$:
{\setlength\abovedisplayskip{1pt}
\setlength\belowdisplayskip{1pt}
\begin{equation}
\mathbb{E}_{x_t \sim \mathcal{D}_t } Dru(z,x_t)= \mathbb{E}_{x_t \sim \mathcal{D}_t } (Var_{\theta_h\sim\theta_{h;k}}(h_{\theta_h}(x_t))).
\label{eqa:DRUf}
\end{equation}}
By analyzing the simplified term $Dru(z)$ of $\mathbb{E}_{x_t \sim \mathcal{D}_t } Dru(z,x_t)$, it is straight-forward that the $i^{th}$ dimension numeric value $Dru(z_i)$ represents the distributional uncertainty of the $i^{th}$ neuron $z_i$ of the encoder representations $z$.
% Obviously,  $Dru(z)$ is also a $d$-dimension vector, where the value of $i$-dimension of  $Dru(z)$, denoted as $Dru(z_i)$  corresponding to the distribution uncertainty of that dimension representations, i.e., $z_i$.
Accordingly, we hypothesize that if $Dru(z_i)$ is \textit{small}, the $i^{th}$ representation $z_i$ induces \textit{little} uncertainty, alternatively robust, to discriminate all target samples and the vice versa. In other words, $Dru(z_i)$ \textit{estimates} the robustness of the $i^{th}$ feature representation to discriminate the target samples. In addition, it can also effectively work as a probe to \textit{compare} the robustness among different feature representation dimensions. To this end, we make our \textit{conjecture} clear: in a very challenging SFUDA task, $Dru(z)$ may be used to assess the transferability of feature representation $z$ to $D_t$ given a pre-trained source domain model.

%that  contains  the distribution uncertainty of $z$ about  all data in $D_t$. 
%As integrated the whole data in $D_t$,  $Dru(z)$ can be regarded as an assessment of $D_t$ to $z$.


%, i.e., can $Dru(z)$  suggest what representations of the source model are more transferable?
%To this end,  we resort the dimension of representation $z$ according to $Dru(z)$ and  then split feature representations  $z$ into two $\mathbb{R}^{ \frac{d}{2}}$ representations:  $z_{low}$ extract $\frac{d}{2}$ dimensions  representations that corresponding to  low $Dru(z)$, while $z_{high}$ extract other  $\frac{d}{2}$  dimensions  representations that with high $Dru(z)$. 
%we split feature representations  $h \in \mathbb{R}^{ d}$ into two $\mathbb{R}^{ \frac{d}{2}}$ representations according to the $Dru(z)$  and investigate their transferability.
%For the source trained feature representations  $h \in \mathbb{R}^{ d}$,  we consider the each dimension of it is an independent representation.
%What we want to show is:  the representations in  $z_{low}$ is  more transferable than  $z_{high}$. The details are as follows.

\underline{\textbf{\textit{Evidence:}}} To verify it, we conduct experiments to study the relationship between the $Dru(z_i)$ and the transferability of $z_i$. To be specific, in Fig.\ref{fig:DRU_transfer}, we compare our measurement $Dru(z)$ with the following cross-domain transferability measurements, \textit{but inapplicable in SFUDA}: 1）the corresponding angle, 2) performance accuracy. Using the Office-Home dataset, we conduct experiments on the following three transfer tasks: Cl$\rightarrow$Ar, Cl$\rightarrow$Pr and Cl$\rightarrow$Re. In this verification, the feature $z \in \mathbb{R}^{ 256}$ is the penultimate layer feature of the ResNet-50 encoder. For each adaptation task, we feedforward all target data to the pre-trained source model and finally calculate $Dru(z)$ as follows: $Dru(z)=[Dru(z_1),Dru(z_2),..., Dru(z_{256})]$. For clarified verification, we split the 256-dim representations $z$ into two separate 128-dim vectors $z_{low}$ and $z_{high}$, representing the ones with the 128 smallest $Dru(z_i)$ and the 128 largest $Dru(z_i)$ respectively. 
% We use a ResNet-50\cite{he2016deep} along with an extra fully connected (fc) layer (256-dim) to extract feature representation $z \in \mathbb{R}^{ 256}$, and a fc layer (65-dim, corresponding to the number of categories of Office-Home) with a weight normalization layer as classifier $g$.
% For each task, we train the source model, then apply it to target domain data and finally calculate the Equation \ref{eqa:DRUf} to get $Dru(z)=[Dru(z_1),Dru(z_2), ..., Dru(z_{256})]$.


\textit{First,} we compare the classification performances on source $D_s$ and target domain $D_t$, using $z_{low}$ and $z_{high}$ as features. % Note, take $z_{low}$ as an example, given the extracted $z$, we only remain its values in $z_{low}$ dimensions and set other dimensions to 0, and then forward it to the classifier to get a prediction. 
In Fig.\ref{fig:DRU_transfer}, it can be seen that for all three adaptation tasks, the prediction using $z_{low}$ is more accurate than $z_{high}$ in target domain $D_T$, indicating that $z_{low}$ with less uncertainties are more transferable than $z_{high}$ to the target domain. 
% \chensays{what?} while is lower than $z_{high}$ in source domain. 
% These results also suggest that $z_{low}$ were more transferable to target domain, while $z_{high}$ overfits more to the source domain. 
We also visualize the semantic information of two neurons with the largest and smallest uncertainty $Dru(z_i)$ respectively in Figure \ref{fig_teaser}.

\textit{Second,} we compare the corresponding angle \cite{chen2019transferability} with $Dru$ as two criterions to quantitatively measure the transferability of $z_{low}$ and $z_{high}$. Specifically, we extract and divide the source and target features to four parts: $H_{s;low}$, $H_{s;high}$, $H_{t;low}$ and $H_{t;high}$ based on the feature positions of $z_{low}$ and $z_{high}$. The corresponding angles are calculated based on \cite{chen2019transferability}. It can be observed that the corresponding angle of $z_{low}$ is larger than that of $z_{high}$, demonstrating that $z_{low}$ has better transferability. 

The experimental observations from the series of studies above verified that $Dru(z)$ calculated on $D_t$ is able to assess the transferability of $z$ to $D_t$. Considering the above properties, we define $-Dru(z)$ as the transferability index of $z$, denoted as $T(z)$. As a benefit, it is useful for SFUDA methods to discover which representations in the source model are more transferable for the target domain in the absence of source data, thus making better use of source domain knowledge. 


% Compared with $z_i$ with high $Dru(z_i)$, the $z_i$ with lower $Dru(z_i)$ is more transferable to target domain $D_t$. 

\subsection{Dru and the Sample Identifiability}
\label{sec:3.3}

We introduce and discuss how Dru is used to approximate and measure the sample identifiability. We follow the previous subsection to discuss the following: the \textit{conjecture} via formula derivation and the \textit{evidence} via experimental results.

\underline{\textbf{\textit{Conjecture:}}} We can also calculate the expectation of $Dru(z,x_t)$ wrt. $z \sim \mathbb{R}^{d}$ to explore the role of $Dru(z,x_t)$ on $x_t$ as follows:
{\setlength\abovedisplayskip{1pt}
\setlength\belowdisplayskip{1pt}
\begin{equation}
\mathbb{E}_{z \sim \mathbb{R}^{d}} Dru(z,x_t)= \mathbb{E}_{h(x_{t})\sim \mathbb{R}^{d}} (Var_{\theta_h\sim\theta_{h;k}}(h_{\theta_h}(x_t))). 
\end{equation}}
% We simplify it as $Dru(x_t)$. 
Integrating on all $z$, $Dru(x_t)$ can be regarded as an overall assessment of the source learned representations $z$ for $x_t$. 

As we train the representations $z$ using source domain data, $z$ implicitly contains the structural information of source domain $D_S$. Therefore, we conjecture that $Dru(x_t)$ can capture the proximity of $x_t$ to the inaccessible source domain data distribution. In the following, we show that  $Dru(x_t)$ is related to the distribution shift of the target input $x_t$ and source data $D_s$. 

\underline{\textbf{\textit{Evidence:}}} Still, we split the target dataset $D_t$ into two parts, where $D_{low}$ collects $x_t$ with small $Dru(x_t)$ (satisfying $Dru(x_t)<mean(\{Dru(x_t)\}_{x_t \in D_t})$), and  $D_{high}$ collects other samples with high $Dru(x_t)$.
We use our source feature extractor $h_{s;\theta_h}$ to extract features, and compare with the well-known $\mathcal{A}$-distance \cite{ben2010theory} and MMD distance \cite{gretton2006kernel} measure the domain discrepancy between $D_{low}$ and $D_s$, and $D_{high}$ and $D_s$ respectively.
In Fig.\ref{fig:DRU_transfer}, it is shown that for both measurements and all three experiments, the discrepancy between $D_s$ and $D_{low}$ is closer to that between $D_{s}$ and $D_{high}$.
The results suggest that $Dru(x_t)$ implicitly reveals $D_s$ and it can capture the domain discrepancy approximately even without the source data.

% We argue that this characteristic is extremely valuable to SFUDA. Many UDA theoretical works \cite{ben2010theory,gretton2006kernel,zhang2019bridging} indicate that the performance of a model on target dataset, is related to its performance on source dataset and the domain discrepancy of the two datasets. In SFUDA, the provide source model is efficient on source dataset. Therefore, $Dru(x_t)$  contains the prediction accuracy information of the model for $x_t $. 

We evaluate the classification accuracy of source model on the $D_{low}$ and $D_{high}$. From the last sub-figure in Figure\ref{fig:DRU_transfer}, it is shown that the accuracy of source model on $D_{low}$ is higher than that on $D_{high}$, indicating the samples on $D_{low}$ are more identifiable and discriminative in target domains.
With the above observations, we define $I(x_t)=\frac{m}{Dru(x_t)}$ as the identifiability index of $x_t$, where $m=mean(\{Dru(x_t)\}_{x_t \in D_t}$.




%DRC focus the uncertainty of the representation  caused by distribution shift.
%\begin{equation}
%\mathbb{E}_{x \sim \mathcal{X}_t } [(h_{\theta_h\sim P(\theta_h|D_s)}(x))
%\end{equation}
%where the $D_S$ and $D_T$ denote the source domain and target domain, $P(\theta_h|D_s)$ is the posterior distribution over parameters given the data in $D_s$, $h_{\theta_h}(x))$ the feature representations of $x$ extracted by encoder $z$ parameterized by $\theta_h$.






%\begin{figure}[t]
%  \centering
  %\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
 
    %\includegraphics[width=0.9\linewidth]{figs/visda.eps}
   
%   \caption{ Performance on different parts \chensays{remember to adjust the font size. otherwise, you will always spend more time in the final day to re-draw the figures.}}
%   \label{fig:acc_curve}
%   \vspace{-6mm}
%\end{figure}

==> samples/uncertainty.tex <==


\begin{figure*}[t]
  \centering
  %\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.24\linewidth]{figs/CA.eps}
    %\includegraphics[width=0.24\linewidth]{figs/CP.eps}
    %\includegraphics[width=0.24\linewidth]{figs/CR.eps}
     \includegraphics[width=0.8\linewidth]{figs/fig_tfs.pdf}
    \vspace{-6mm}
   \caption{The experiment of the source trained model on three source$\rightarrow$target tasks: Cl$\rightarrow$Ar, Cl$\rightarrow$Pr and Cl$\rightarrow$Re. The first  figures show the performance of two different representations $z_{low}$ and $z_{high}$ on target domain. The second figure compares the corresponding angle between $z_{low}$ and $z_{high}$. The third and fource  figures calculate the MMD distance and \mathcal{A}-distance between $D_{low}$ and $D_s$, and $D_{high}$ and $D_s$. The last figure show the performance of the model on the  $D_{low}$ and $D_{high}$. }
   \label{fig:DRU_transfer}
   \vspace{-6mm}
\end{figure*}

%In domain adaptation, transferability characterizes the ability of feature representations to bridge the discrepancy across domains\cite{chen2019transferability}, which is also referred to as the invariance of the learned representations across domains\cite{chen2020harmonizing}.
%It is the key to effectively transferring a learning model from the source domain to the target domain via the feature representations.
%Many vanilla UDA methods used to measure the domain discrepancy between features from source and target domain, such as A-distance, H-distance and discrepancy distance, can be regarded as measures of transferability of the feature representations \cite{ibrahim2021newer}. 
%Recently, \cite{chen2019transferability} propose a corresponding angle to explicitly investigate the transferability of feature representations. 
%Previous works in measuring transferability require  a well-trained model in the source domain and labeled target domain data \cite{nguyen2020leep,bao2019information}.
%These vanilla UDA methods, however,  require  to extract the representations of the source data and target data simultaneously, which are not available in SFUDA.
%Although these methods have shown their effectiveness in vanilla UDA, they are unapplicable to SFUDA since they need to extract source features from source data.

%Inspired by \cite{gao2020reducing} which describes the domain discrepancy as to the distributional uncertainty between source and target, we propose to study the transferability of the feature representations through their distributional uncertainty.
%In the following, we model the distributional uncertainty of the representations (Dru), and experimentally analyze its relationship to feature transferability.
%However, in SFUDA, we cannot get the features of the source domain data.
%Therefore, measure the transferability of the representation by compare its extracted features on the two domains is infeasible.
%Inspired by the definition, we rethink the transferability as the robustness of the representation learned from source domain on target domain.
%The robustness, according to \cite{kwon2021repurposing}, can be captured by the uncertainty.
%Although the source data is not available, SFUDA provide a well-trained model in the source domain, which means the information about source domain is embedded on the model. 
%Different from vanilla UDA.
%\subsection{}
%

\subsection{The Dru Model}
\label{sec:Dru}

In this paper, we focus on the K-way visual object classification task. 
We denote the labeled source domain data as $D_s=\{(x_i^s,y_i^s)\}_{i=1}^{n_s}$, where $x_s \in \mathcal{X}_s$, $y_s \in \mathcal{Y}_s$, and $n_s$ is the number of samples. A source model $f_s: \mathcal{X}_s \rightarrow \mathcal{Y}_s$ is trained, parameterized by $f_{s;\theta}=g_{s;\theta_g} \circ h_{s;\theta_h}$, where $h_{s;\theta_h}$ is the feature extractor  parameterized by $\theta_h$ to  embed the input into feature representations $z$,  and $g_{s;\theta_g}$ is the classifier  parameterized by  $\theta_g$. 
The unlabeled target domain $D_t=\{x_i^t\}_{i=1}^{n_t}$ consists of $n_t$ samples and $x_t \in \mathcal{X}_t$. 
 
Given a target sample $(x_t,y_t)$, :
{\setlength\abovedisplayskip{1pt}
\setlength\belowdisplayskip{1pt}
\begin{equation}
P(y_t|x_t,D_s)= \iint \underbrace {P(y_t|\mu)}_{Data} \underbrace {P(\mu|x_t,\theta)}_{Distributional} \underbrace {P(\theta|D_s)}_{Model}d\theta d\mu,
\label{eqa:uncertainty}
\end{equation}}
where $\mu=g_{s;\theta_g} \circ z$ denotes the prediction of the model which relies on the extracted feature representation $z$ and classifier $g_{s;\theta_g}$. 
The ``distributional uncertainty'' is presented by the distributional part in Equation \ref{eqa:uncertainty}, which refers to the uncertainty on prediction that arises from whether the input data $x_t$ is fat from training distribution $D_s$. The other two parts -- the ``data uncertainty'' and ``model uncertainty'', 
capture the uncertainty from input data and model parameters respectively.
The detailed explanations of the two uncertainties can be found in \cite{malinin2018predictive,gawlikowski2021survey,nandy2020towards}.
%The distributional uncertainty of this target samples can be captured from $\iint  P(\mu|x_t,\theta)  P(\theta|D_s) d\mu d\theta.$

Inspired by the argument that the optimal target classifier is closely related to the source one \cite{kuzborskij2013stability, liang2020we}, we assume it effective to \textit{re-use and fix} the source classifier parameter, that is able to reasonably fit the target data well.
% is efficient for the target domain and regard classifier parameters as fixed values. 
Then we replace $\mu$ and $\theta$ in Equation \ref{eqa:uncertainty} by the feature representation $z$ and the feature extractor $\theta_h$ respectively and re-formulate the Equation \ref{eqa:uncertainty} as follows: 
{\setlength\abovedisplayskip{1pt}
\setlength\belowdisplayskip{1pt}
\begin{equation}
 P(y_t|x_t,D_s)=\iint P(y_t|z) P(z|x_t,\theta_h)  P(\theta_h|D_s)d\theta_h.
\end{equation}}
As the distributional uncertainty $P(z|x_t,\theta_h)$ is conditioned on both the target input $x_t$ and the encoder parameters $\theta_h$, its calculation inevitably accompanies the “model uncertainty'' from $ P(\theta_h|D_s)$. However, as SFUDA assumes that the source model performs well on the source domain, we argue in this paper the “model uncertainty'' is very small and can be ignored. 
% However, it is obvious that term is conditioned on $\theta_h$. Calculating  its uncertainty  inevitably accompanied “model uncertainty'' from $ P(\theta_h|D_s)$.
% Fortunately, SFUDA assume that the source model is “well-trained'' on the source domain. In this case, the “model uncertainty'' is very small and can be ignored. 
Therefore, we can explicitly measure the uncertainty $P(z|x_t,\theta_h)$ to approximate the distributional uncertainty of the feature representations --- note that we denote it as Dru in the following to simplify.
%Thus we can estimate the Dru by directly measuring the uncertainty in Equation \ref{eqa:Dru}.

Out of various methods to measure the uncertainty \cite{kendall2017uncertainties,gal2016dropout,lakshminarayanan2016simple}, we adopt the sensitivity analysis variant \cite{nagy2007distributional} in this paper for computational efficacy. To be specific, $K$ model parameter sets $\{\theta_{h;k}=(1+r_k)*\theta_h\}_{k=1}^K$ are \textit{firstly} calculated by inserting $K$ random perturbations $\{r_k\}_{k=1}^K$ and \textit{then} the uncertainty is estimated by calculating the variance of the $K$ outputs.
% it adds perturbations $\{r_k\}_{k=1}^K$ to the model parameters to obtain multiple $\{\theta_{h;k}=(1+r_k)*\theta_h\}_{k=1}^K$ and estimate uncertainty by the variance of their output.
% \chensays{I suggest putting the following in the implementation details or supplement; but it is your choice. In this paper, $r$ is randomly sampled from $U(-0.05,0.05)$, and $k$ is set to 2.}
% sensitivity analysis \cite{nagy2007distributional} that add perturbations $\{r_k\}_{k=1}^K$ to the model parameter to get multiple $\{\theta_{h;k}=(1+r_k)*\theta_h\}_{k=1}^K$ and estimate uncertainty by the variance of their output. In this paper, $r$ is randomly sampled from $U(-0.05,0.05)$, and $k$ is set to 2.
To summarize, for any $x_t, z$, the Dru can be calculated by the following:
{\setlength\abovedisplayskip{1pt}
\setlength\belowdisplayskip{1pt}
\begin{equation}
  Dru(z,x_t)= Var_{\theta_h\sim\theta_{h;k}}(h_{\theta_h}(x_t)). 
  \label{eqa:esDRU}
  \vspace{-3mm}
\end{equation}}
%After integrating $x_t$ on the whole dataset $D_t$, we can obtain the Dru by compute the uncertainty in: 
%{\setlength\abovedisplayskip{1pt}
%\setlength\belowdisplayskip{1pt}
%\begin{equation}
% \mathbb{E}_{x_t \sim D_t} P(h|x_t,\theta_h).
% \label{eqa:Dru}
%\end{equation}}
% \vspace{-3mm}

From Equation \ref{eqa:esDRU}, as Dru is related to two variables $z$ and $x_t$, thus inspiring two ways to understand it. They are discussed in the following two subsections, forming and introducing a new measurement for SFUDA. 

\subsection{Dru and the Representation Transferability}
\label{sec:3.2}
% \vspace{-1mm}
% From Equation \ref{eqa:esDRU}, we see Dru is related to two variables $z$ and $x_t$, which provide us two ways to understand it.
In this subsection, we introduce and discuss how Dru is used to approximate and measure the representation transferability. The following discussion comprises two parts: the \textit{conjecture} via formula derivation and the \textit{evidence} via experimental results.

\underline{\textbf{\textit{Conjecture:}}} To investigate the effect of Dru on the representation $z$, we propose to calculate the expectation of $D(z,x_t)$ by integrating $x_t$ over the target domain $D_t$:
{\setlength\abovedisplayskip{1pt}
\setlength\belowdisplayskip{1pt}
\begin{equation}
\mathbb{E}_{x_t \sim \mathcal{D}_t } Dru(z,x_t)= \mathbb{E}_{x_t \sim \mathcal{D}_t } (Var_{\theta_h\sim\theta_{h;k}}(h_{\theta_h}(x_t))).
\label{eqa:DRUf}
\end{equation}}
By analyzing the simplified term $Dru(z)$ of $\mathbb{E}_{x_t \sim \mathcal{D}_t } Dru(z,x_t)$, it is straight-forward that the $i^{th}$ dimension numeric value $Dru(z_i)$ represents the distributional uncertainty of the $i^{th}$ neuron $z_i$ of the encoder representations $z$.
% Obviously,  $Dru(z)$ is also a $d$-dimension vector, where the value of $i$-dimension of  $Dru(z)$, denoted as $Dru(z_i)$  corresponding to the distribution uncertainty of that dimension representations, i.e., $z_i$.
Accordingly, we hypothesize that if $Dru(z_i)$ is \textit{small}, the $i^{th}$ representation $z_i$ induces \textit{little} uncertainty, alternatively robust, to discriminate all target samples and the vice versa. In other words, $Dru(z_i)$ \textit{estimates} the robustness of the $i^{th}$ feature representation to discriminate the target samples. In addition, it can also effectively work as a probe to \textit{compare} the robustness among different feature representation dimensions. To this end, we make our \textit{conjecture} clear: in a very challenging SFUDA task, $Dru(z)$ may be used to assess the transferability of feature representation $z$ to $D_t$ given a pre-trained source domain model.

%that  contains  the distribution uncertainty of $z$ about  all data in $D_t$. 
%As integrated the whole data in $D_t$,  $Dru(z)$ can be regarded as an assessment of $D_t$ to $z$.


%, i.e., can $Dru(z)$  suggest what representations of the source model are more transferable?
%To this end,  we resort the dimension of representation $z$ according to $Dru(z)$ and  then split feature representations  $z$ into two $\mathbb{R}^{ \frac{d}{2}}$ representations:  $z_{low}$ extract $\frac{d}{2}$ dimensions  representations that corresponding to  low $Dru(z)$, while $z_{high}$ extract other  $\frac{d}{2}$  dimensions  representations that with high $Dru(z)$. 
%we split feature representations  $h \in \mathbb{R}^{ d}$ into two $\mathbb{R}^{ \frac{d}{2}}$ representations according to the $Dru(z)$  and investigate their transferability.
%For the source trained feature representations  $h \in \mathbb{R}^{ d}$,  we consider the each dimension of it is an independent representation.
%What we want to show is:  the representations in  $z_{low}$ is  more transferable than  $z_{high}$. The details are as follows.

\underline{\textbf{\textit{Evidence:}}} To verify it, we conduct experiments to study the relationship between the $Dru(z_i)$ and the transferability of $z_i$. To be specific, in Fig.\ref{fig:DRU_transfer}, we compare our measurement $Dru(z)$ with the following cross-domain transferability measurements, \textit{but inapplicable in SFUDA}: 1）the corresponding angle, 2) performance accuracy. Using the Office-Home dataset, we conduct experiments on the following three transfer tasks: Cl$\rightarrow$Ar, Cl$\rightarrow$Pr and Cl$\rightarrow$Re. In this verification, the feature $z \in \mathbb{R}^{ 256}$ is the penultimate layer feature of the ResNet-50 encoder. For each adaptation task, we feedforward all target data to the pre-trained source model and finally calculate $Dru(z)$ as follows: $Dru(z)=[Dru(z_1),Dru(z_2),..., Dru(z_{256})]$. For clarified verification, we split the 256-dim representations $z$ into two separate 128-dim vectors $z_{low}$ and $z_{high}$, representing the ones with the 128 smallest $Dru(z_i)$ and the 128 largest $Dru(z_i)$ respectively. 
% We use a ResNet-50\cite{he2016deep} along with an extra fully connected (fc) layer (256-dim) to extract feature representation $z \in \mathbb{R}^{ 256}$, and a fc layer (65-dim, corresponding to the number of categories of Office-Home) with a weight normalization layer as classifier $g$.
% For each task, we train the source model, then apply it to target domain data and finally calculate the Equation \ref{eqa:DRUf} to get $Dru(z)=[Dru(z_1),Dru(z_2), ..., Dru(z_{256})]$.


\textit{First,} we compare the classification performances on source $D_s$ and target domain $D_t$, using $z_{low}$ and $z_{high}$ as features. % Note, take $z_{low}$ as an example, given the extracted $z$, we only remain its values in $z_{low}$ dimensions and set other dimensions to 0, and then forward it to the classifier to get a prediction. 
In Fig.\ref{fig:DRU_transfer}, it can be seen that for all three adaptation tasks, the prediction using $z_{low}$ is more accurate than $z_{high}$ in target domain $D_T$, indicating that $z_{low}$ with less uncertainties are more transferable than $z_{high}$ to the target domain. 
% \chensays{what?} while is lower than $z_{high}$ in source domain. 
% These results also suggest that $z_{low}$ were more transferable to target domain, while $z_{high}$ overfits more to the source domain. 
We also visualize the semantic information of two neurons with the largest and smallest uncertainty $Dru(z_i)$ respectively in Figure \ref{fig_teaser}.

\textit{Second,} we compare the corresponding angle \cite{chen2019transferability} with $Dru$ as two criterions to quantitatively measure the transferability of $z_{low}$ and $z_{high}$. Specifically, we extract and divide the source and target features to four parts: $H_{s;low}$, $H_{s;high}$, $H_{t;low}$ and $H_{t;high}$ based on the feature positions of $z_{low}$ and $z_{high}$. The corresponding angles are calculated based on \cite{chen2019transferability}. It can be observed that the corresponding angle of $z_{low}$ is larger than that of $z_{high}$, demonstrating that $z_{low}$ has better transferability. 

The experimental observations from the series of studies above verified that $Dru(z)$ calculated on $D_t$ is able to assess the transferability of $z$ to $D_t$. Considering the above properties, we define $-Dru(z)}$ as the transferability index of $z$, denoted as $T(z)$. As a benefit, it is useful for SFUDA methods to discover which representations in the source model are more transferable for the target domain in the absence of source data, thus making better use of source domain knowledge. 


% Compared with $z_i$ with high $Dru(z_i)$, the $z_i$ with lower $Dru(z_i)$ is more transferable to target domain $D_t$. 

\subsection{Dru and the Sample Identifiability}
\label{sec:3.3}

We introduce and discuss how Dru is used to approximate and measure the sample identifiability. We follow the previous subsection to discuss the following: the \textit{conjecture} via formula derivation and the \textit{evidence} via experimental results.

\underline{\textbf{\textit{Conjecture:}}} We can also calculate the expectation of $Dru(z,x_t)$ wrt. $z \sim \mathbb{R}^{d}$ to explore the role of $Dru(z,x_t)$ on $x_t$ as follows:
{\setlength\abovedisplayskip{1pt}
\setlength\belowdisplayskip{1pt}
\begin{equation}
\mathbb{E}_{z \sim \mathbb{R}^{d}} Dru(z,x_t)= \mathbb{E}_{h(x_{t})\sim \mathbb{R}^{d}} (Var_{\theta_h\sim\theta_{h;k}}(h_{\theta_h}(x_t))). 
\end{equation}}
% We simplify it as $Dru(x_t)$. 
Integrating on all $z$, $Dru(x_t)$ can be regarded as an overall assessment of the source learned representations $z$ for $x_t$. 

As we train the representations $z$ using source domain data, $z$ implicitly contains the structural information of source domain $D_S$. Therefore, we conjecture that $Dru(x_t)$ can capture the proximity of $x_t$ to the inaccessible source domain data distribution. In the following, we show that  $Dru(x_t)$ is related to the distribution shift of the target input $x_t$ and source data $D_s$. 

\underline{\textbf{\textit{Evidence:}}} Still, we split the target dataset $D_t$ into two parts, where $D_{low}$ collects $x_t$ with small $Dru(x_t)$ (satisfying $Dru(x_t)<mean(\{Dru(x_t)\}_{x_t \in D_t})$), and  $D_{high}$ collects other samples with high $Dru(x_t)$.
We use our source feature extractor $h_{s;\theta_h}$ to extract features, and compare with the well-known $\mathcal{A}$-distance \cite{ben2010theory} and MMD distance \cite{gretton2006kernel} measure the domain discrepancy between $D_{low}$ and $D_s$, and $D_{high}$ and $D_s$ respectively.
In Fig.\ref{fig:DRU_transfer}, it is shown that for both measurements and all three experiments, the discrepancy between $D_s$ and $D_{low}$ is closer to that between $D_{s}$ and $D_{high}$.
The results suggest that $Dru(x_t)$ implicitly reveals $D_s$ and it can capture the domain discrepancy approximately even without the source data.

% We argue that this characteristic is extremely valuable to SFUDA. Many UDA theoretical works \cite{ben2010theory,gretton2006kernel,zhang2019bridging} indicate that the performance of a model on target dataset, is related to its performance on source dataset and the domain discrepancy of the two datasets. In SFUDA, the provide source model is efficient on source dataset. Therefore, $Dru(x_t)$  contains the prediction accuracy information of the model for $x_t $. 

We evaluate the classification accuracy of source model on the $D_{low}$ and $D_{high}$. From the last sub-figure in Figure\ref{fig:DRU_transfer}, it is shown that the accuracy of source model on $D_{low}$ is higher than that on $D_{high}$, indicating the samples on $D_{low}$ are more identifiable and discriminative in target domains.
With the above observations, we define $I(x_t)=\frac{m}{Dru(x_t)}$ as the identifiability index of $x_t$, where $m=mean(\{Dru(x_t)\}_{x_t \in D_t}$.




%DRC focus the uncertainty of the representation  caused by distribution shift.
%\begin{equation}
%\mathbb{E}_{x \sim \mathcal{X}_t } [(h_{\theta_h\sim P(\theta_h|D_s)}(x))
%\end{equation}
%where the $D_S$ and $D_T$ denote the source domain and target domain, $P(\theta_h|D_s)$ is the posterior distribution over parameters given the data in $D_s$, $h_{\theta_h}(x))$ the feature representations of $x$ extracted by encoder $z$ parameterized by $\theta_h$.






%\begin{figure}[t]
%  \centering
  %\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
 
    %\includegraphics[width=0.9\linewidth]{figs/visda.eps}
   
%   \caption{ Performance on different parts \chensays{remember to adjust the font size. otherwise, you will always spend more time in the final day to re-draw the figures.}}
%   \label{fig:acc_curve}
%   \vspace{-6mm}
%\end{figure}

==> tables/tab_transferability.tex <==
\begin{table}

\caption{Comparison with existing transferability measurements on three office-home tasks Cl$\rightarrow$Ar, Cl$\rightarrow$Pr and Cl$\rightarrow$Re. $z_{low}$ and $z_{high}$  are features with  low $UTR_D$ and  high $UTR_D$, respectively. The $\uparrow$/$\downarrow$ indicates the larger/smaller the value, the higher the transferability. 
In each task, current transferability measurements are calculated on $Z_{low}$ and $Z_{high}$, respectively.
The more transferable one is bolded.}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|cc|cc|cc}

\hline
\multirow{2}{*}{Measurement}&\multicolumn{2}{c}{Cl$\rightarrow$Ar}\vline&\multicolumn{2}{c}{Cl$\rightarrow$Pr}\vline&\multicolumn{2}{c}{Cl$\rightarrow$Re}\\
%\cmidrule(r){2-3}\cmidrule(r){4-5}\cmidrule(r){6-7}
& $Z_{low}$ & $Z_{high}$& $Z_{low}$ & $Z_{high}$& $Z_{low}$ & $Z_{high}$\\
\hline
%source-only &44.6& 67.3 &74.0\\
%$\lambda_1$ &0.5/78.7 &2/79.5&5/81.2 &10/78.0 &15/77.2&25/75.7  \\
%$\lambda_2$ &0.03/75.8 &0.1/77.7&0.3/80.4 &1/81.2 &3/80.4&10/68.6  \\

MMD$\downarrow$&\textbf{0.71}&0.74&\textbf{0.20}&0.21&\textbf{0.17}&0.18 \\
A-Distance$\downarrow$&\textbf{1.40}&1.43&\textbf{1.20}&1.25&\textbf{1.40}&1.44 \\
Corresponding Angle$\uparrow$ &\textbf{0.97}&0.94 &\textbf{0.98}&0.97&\textbf{0.99}&0.97\\
LogMe$\uparrow$&\textbf{0.85}&0.81 &\textbf{0.84}&0.82& \textbf{0.84}&0.81\\
LEEP$\uparrow$&\textbf{-2.81}&-2.98 &\textbf{-2.39}&-2.65& \textbf{-2.38}&-2.54\\
NCE$\uparrow$&\textbf{-1.71}&-1.99 &\textbf{-1.43}&-1.58& -1.44&\textbf{-1.43}\\
%Accuracy$\uparrow$&\textbf{45.5\%}&42.2\%&\textbf{66.4\%}&64.2\%&\textbf{73.9\%}&70.5\%\\
%$\lambda_1$ &0.03/79.5 &0.05/80.8&0.08/81.2 &0.12/81.0 &0.2/78.8&0.3/78.6  \\
%$\lambda_2$ &0.03/79.5 &0.05/80.8&0.08/81.2 &0.12/81.0 &0.2/78.8&0.3/78.6  \\
\hline
\end{tabular}}

\label{tab_transferability}

\end{table}


==> tables/tab_unc.tex <==
\begin{table}[t]\scriptsize
\caption{Performance(\%) with different uncertainty estimations.}
\centering
\begin{tabular}{l|c|c|c}
\hline
Method &Ar$\rightarrow$Cl &Ar$\rightarrow$Pr &Ar$\rightarrow$Re\\
\hline
%source-only &44.6& 67.3 &74.0\\
Sensitive &59.8 &81.2&83.2  \\
Ensemble &59.1&80.7&82.9\\
MC dropout &59.3&80.5&82.7\\
\hline
\end{tabular}

\label{tab_abl_uncer}

\end{table}
